APIDocBooster: An Extract-Then-Abstract Framework Leveraging Large Language Models for Augmenting API Documentation

API documentation is often the most trusted resource for programming. Many approaches have been proposed to augment API documentation by summarizing complementary information from external resources such as Stack Overflow. Existing extractive-based summarization approaches excel in producing faithful summaries that accurately represent the source content without input length restrictions. Nevertheless, they suffer from inherent readability limitations. On the other hand, our empirical study on the abstractive-based summarization method, i.e., GPT-4, reveals that GPT-4 can generate coherent and concise summaries but presents limitations in terms of informativeness and faithfulness. We introduce APIDocBooster, an extract-then-abstract framework that seamlessly fuses the advantages of both extractive (i.e., enabling faithful summaries without length limitation) and abstractive summarization (i.e., producing coherent and concise summaries). APIDocBooster consists of two stages: (1) \textbf{C}ontext-aware \textbf{S}entence \textbf{S}ection \textbf{C}lassification (CSSC) and (2) \textbf{UP}date \textbf{SUM}marization (UPSUM). CSSC classifies API-relevant information collected from multiple sources into API documentation sections. UPSUM first generates extractive summaries distinct from the original API documentation and then generates abstractive summaries guided by extractive summaries through in-context learning. To enable automatic evaluation of APIDocBooster, we construct the first dataset for API document augmentation. Our automatic evaluation results reveal that each stage in APIDocBooster outperforms its baselines by a large margin. Our human evaluation also demonstrates the superiority of APIDocBooster over GPT-4 and shows that it improves informativeness, relevance, and faithfulness by 13.89\%, 15.15\%, and 30.56\%, respectively.

==> bench.tex <==
We craft \bench{}, the first benchmark to evaluate approaches for augmenting API documentation from multiple sources. 
% In addition, we cluster consecutive context-dependent sentences together to form the semantic unit, making \bench available for the classification task of identifying context-dependent sentences.
% \bench consists of two-stage labeling processes.
Figure~\ref{fig:bench} illustrates the construction process of \bench{} with two main steps, data collection and labeling process.
% \textcolor{blue}{Jiakun suggests deleting below two paragraphs since its redundant.}\bowen{I have removed the redundant part.}
In the data collection step, we prepare the initial labeling materials by randomly sampling APIs in two popular programming languages. 
We then collect relevant Stack Overflow posts and YouTube videos for each sampled API and pre-process them to produce annotation units (AUs). 
Each AU consists of a certain API and a set of sentences extracted from the relevant YouTube video captions (i.e., the text that is spoken in the video) and Stack Overflow answers.
Then, we perform a two-stage labeling process for each AU. 
In the first stage, annotators cluster contextual sentences and link sentences to their corresponding API documentation sections or indicate that they are API-irrelevant. 
% The first stage output is 4,344 sentences labeled with corresponding API documentation sections. 
In the second stage, annotators create one summary (i.e., a subset of the relevant sentences associated with this section) for each API documentation section from the output of the first stage by considering the requirements mentioned in Section~\ref{sec:task}. 
% Annotators are required to consider the redundancy between the candidate sentences and the original API document.
% The second-stage output consists of 48 summaries for augmenting the original API documentation.
% }


% \begin{figure}
%     \centering
%     \includegraphics[width=1\columnwidth]{figure/benchmark_diagram_v2.pdf}
%     % \vspace{-6mm}
%     \caption{Benchmark construction process. 
%     % (1) we sample APIs and collect relevant online resources from multiple sources to produce annotation units (Section~\ref{sec:benchmark_data_collection}). (2) we perform two-phase labeling to produce human-generated summaries for augmenting API documentation (Section~\ref{sec:labelingprocess}).
%     }
%     \label{fig:bench}
%     % \vspace{-5mm}
% \end{figure}

\subsection{Collecting Annotation Units}
\label{sec:benchmark_data_collection}
% We sample APIs from Python and Java libraries.
% For each sampled API, we automatically collect its potentially relevant \so posts as well as YouTube videos, which is followed by a manual filter.
% Next, we pre-process the data and produce AUs. 

\subsubsection{Collecting APIs}
Following existing approaches~\cite{chengran2022answer, uddin2017automatic}, we collect APIs from Java and Python libraries. 
Specifically, we collect APIs from the \pt~\cite{pytorch} and Android~\cite{android} platform libraries. 
PyTorch is a popular tensor library for deep learning projects. 
The Android platform library consists of APIs to build Android apps. 
We focus on method-level APIs in this benchmark, while our approach applies to multi-level APIs. 
We obtain all method-level APIs of both libraries through web crawling and text parsing techniques. 
% Meanwhile, we observe some APIs with the same method name but different fully qualified names. 
% As PyTorch APIs typically link to the same document page (e.g., torch.nn.functional.tanh\footnote{\url{https://pytorch.org/docs/stable/generated/torch.nn.functional.tanh.html?highlight=tanh\#torch.nn.functional.tanh}} and torch.nn.Tanh\footnote{\url{https://pytorch.org/docs/stable/generated/torch.nn.Tanh.html\#torch.nn.Tanh}}), we keep only one of them.
% \jkl{show an example here.}
% \jkl{I say it is a mixture because the sentences before are related to extracting data. The following sentences are related to filtering data using another data source (i.e., SO here). It might confuse others.}
Since the quality of the API documentation pages varies~\cite{khan2021automatic}, we focus on APIs that greatly need augmentation. 
Considering the APIs which are frequently mentioned in \so indicate whose documentations have more need to be improved~\cite{parnin2012crowd},
we count the occurrences of each API in posts tagged with the API library name and its synonyms~\cite{tagsynonyms} (e.g., \textit{pytorch} and \textit{pytorch-gpu})
.
Then we drop the APIs that have not been mentioned on Stack Overflow.
% Note that we use the API method name rather than the fully qualified name.
% Relaxed search criteria allow us to better find rarely mentioned APIs in \so due to API ambiguity.
% .\jkl{If you mention it here, you may need to show how you count.}
% Specifically, we perform an exact match for each API in all posts tagged with API library name and its synonyms labels. \jkl{example?}
% \so posts are extracted from the official \so data dump.\footnote{https://archive.org/details/stackexchange}
Finally, we randomly sample 10 \pt APIs and 10 Android APIs.

\subsubsection{Automatically Collecting of Resources}

To extract the potentially relevant Stack Overflow posts, we automatically call the Stack Exchange API~\cite{stackexchange}. 
We search with the query $library\_name + API\_name$ to obtain the top 50 relevant \so answers.
%  by using the \so built-in search engine. 
We select the answer if 1) it has a positive score and 2) it contains a natural language description.
% 4) the question post should be tagged with the corresponding library name. 
For each API, we pick the top 50 \so answers; in total,  1,000 ($20 \times 50$) answers are collected.

To obtain the potentially relevant YouTube videos, we use the official YouTube API~\cite{youtubeapi} to automatically search for relevant videos with the same query as for \so search.
As YouTube video data is even scarcer compared to \so posts, we further search with the query $ class\_name + API\_name$ to obtain videos. 
For each query, we extract the top 100 videos for one API, in total 2,000 videos are collected.
Next, we extract video captions to leverage the information in YouTube videos and augment the textual API documents.
We observe that automatically generated captions have no punctuation, thus causing those captions to be unable to be naturally split into sentences.
Therefore, we only consider videos with manually crafted captions. We apply the youtube-transcript-api tool~\cite{transcript} to identify videos with manual captions.
% When extracting captions from candidate YouTube videos, we observe that not all YouTube videos contain the manual captions. Many of video captions are automatically generated. The generated captions have no punctuation, thus those captions are unable to be naturally subdivided into sentences. Considering that dividing those captions into sentences by text spliting tool may result in semantically incomplete sentences or sentences with factual errors, we consider only captions that are manually crafted. Thus we apply youtube-transcript-api tool\footnote{https://pypi.org/project/youtube-transcript-api/} to identify videos that have manual captions and extract their captions. 
Finally, we collect 146 videos with manually crafted captions.

% \subsubsection{Automatically Collecting Augmented Resources}
\subsubsection{Manual Filtering of Resources}
We observe that automatically collected data may still be factually irrelevant to the target API due to the limitation of the search engines.
For example, some data points relevant to TensorFlow API are incorrectly considered related to PyTorch API by the search engine.
Thus, we perform a manual filter to omit irrelevant data and mitigate the threat of API ambiguity. 
% Following TechSumBot, we select the top 10 raw resources from each source for each API.
The first author manually checks the data and picks the top ten \so answers and YouTube videos related to the target API.
The first author focuses on identifying whether the data relates to the target API.
% Note that as long as the data contain target API information, we keep it even if it includes non-target libraries' information.
% Labelers must identify whether each sentence's information is relevant to the target library in the subsequent labeling process.
% , e.g., we need to filter out the data about APIs with the same method name as the target API but in the different class or library. \red{statistis is required.}
Finally, 189 \so answers and 84 YouTube videos are collected.

\subsubsection{Pre-processing Data}

After obtaining \so answers and video captions related to specific APIs, we pre-process the data and produce \textbf{A}nnotation \textbf{U}nits (AUs). 
% Each annotation unit consists of a specific API and multiple relevant sentences from \so answers and video captions. 
First, we use NLTK~\cite{NLTK} to break each text content into sentences. 
We then apply several heuristic rules to reduce data noise. 

For \so answers, we replace hyperlinks, code snippets, tables, and pictures with placeholders.
We keep inline code. 
% Furthermore, We insert a paragraph mark at the end of each answer paragraph to remind labelers.
% We also provide the original question title, link, and description for each answer sentence. 
For YouTube videos, we observe that long video captions commonly contain many irrelevant sentences.
% Some videos focus on the target API only for a certain period of time. 
% In our guideline refinement stage, the average number of sentences for YouTube videos is 553, but the number of insight sentences is 11.9.
% (e.g., some video captions have more than one thousand sentence but less than 100 are relevant to the target API). 
Meanwhile, we observe that sentences and their context sentences that contain name entities in \doc (e.g., API name and API parameters) are usually insight sentences.
% insightful sentences in video captions usually contain name entities in \doc (e.g., API name and API parameters) or are the context of the video captions sentences that contain name entities.}
Thus, we leverage the BM25~\cite{robertson2009probabilistic} algorithm to remove caption sentences irrelevant to the target API coarsely. 
BM25 is a ranking function that is used to estimate the relevance between a given query and a document. Formally, given a query $Q$, the relevance score is given by:
\begin{equation}
% \small
    Score(Q,d)=\sum_{i}^{n}IDF_{q_{i}}\frac{h(q_{i},d)*(k_{1}+1)}{h(q_{i},d)+k_{1}*(1-b+b*\frac{\left | D \right |}{avgdl})}
\end{equation}
\noindent where $q_{i}$ is the $i^{th}$ word in the query $Q$, $h(q_{i},d)$ indicates the frequency of $q_{i}$ occurring in the document $d$, $avgdl$ is the \textbf{a}\textbf{v}era\textbf{g}e \textbf{d}ocument \textbf{l}ength in the text collection, $k_{1}$ and b are adjustable parameters (by default $k_{1}=1.2$ and $b=0.75$, following Robertson et al.~\cite{robertson2009probabilistic}), and $\left | D \right |$ is the length of the document in terms of words. The $IDF(q_{i})$ is the IDF value of $q_{i}$. 
We set each caption sentence as $d$ and manually construct the query for each API as ``API name, hyper-parameter names, type of input and output''. 
We refer to the original API documents for hyper-parameter, input, and output names.
We calculate the ranking score of each caption sentence with respect to the query and select all sentences that have a positive score. In addition, we also include one preceding sentence and one following sentence of the positive score sentence as candidates.
Finally, 5,414 sentences related to 20 APIs are collected to produce 20 AUs. 
Each AU consists of a particular API and a set of sentences extracted from the relevant YouTube video captions and Stack Overflow answers.
% In each AU, there are 131.7 relevant \so answer sentences on average and 139 YouTube video caption sentences on average related to a specific API.
% All \so answer sentences are presented in a text file as well as their question title, \so link, and question description. We also present video caption data in a text file including selected caption sentences, video titles, YouTube links, and video abstracts.
% For \so, we first select the top 50 questions for each API. One annotator manually checks the questions that are relevant to the API and select the top 10-15 answers.

% \red{statistic is required maybe}

\subsection{Labeling Process}
\label{sec:labelingprocess}
Following prior works~\cite{chengran2022answer, angelidis2018summarizing},
we perform a two-phase labeling. 
Five participants are involved in the labeling process, i.e. the first author of the paper (i.e., a1), 
two Ph.D. students (i.e., s1, s2), and two postdoctoral fellows (i.e., p1, p2). 
All annotators have at least two years of programming experience in Java or Python. 
% In the first labeling stage, annotators cluster the semantically-relevant sentences together and classify sentences into API document blocks (as defined in Section~\ref{sec:apiblockclassifier}).
% In the second stage, given each API block, annotators select sentences to form an extractive summary while taking into account the redundancy between generated summaries and original API documentation.
% Annotators should take into account sentences' clarity, representativeness, redundancy among all the candidates, and redundancy to the original API document. 
% Note that, for each labeling stage, we perform an iterative guideline refinement process and validation labeling to improve the annotators' agreement.

\subsubsection{Phase 1: API Documentation Section Classification}
\label{sentclassfier}

% In this stage, annotators need to identify the insightful sentences for the target API and classify them into API specifications. 
Given sentences extracted from API-relevant \so answers and YouTube videos, annotators 1) cluster semantically relevant sentences together and 
2) specify the API documentation sections that the sentences belong to.

One novelty of \bench is context awareness.
Since we observe that some sentences require context to be understood,
we ask annotators to label both API documentation sections and the context dependence of each sentence \cite{treude2016augmenting}. 
% However, existing related datasets~\cite {wang2019extracting,uddin2017automatic} neglect the context of sentences.
% We show an example randomly extracted from a dataset proposed by DEEPTip~\cite{wang2019extracting}. 
% This dataset contains \so sentences labeled as tips or not for PHP APIs.  
% One sentence, i.e., ``however, it will not allow you to bind any data to the executed sql.'' is labeled as a tip in the dataset.\footnote{\url{https://github.com/DEEPTIPExtraction/DEEPTip/blob/master/dataset/sent_tip.pos}}
% Without providing the context, it is hard to determine which API does not allow data binding to the SQL.
% However, we can easily identify the API by providing the context along with the current sentence\footnote{\url{https://stackoverflow.com/a/38553989/10143020}}, i.e., ``Alternatively, you can use $\textbf{conn->exec}$(sql), which works regardless. However, it will not allow you to bind any data to the executed SQL.''
% Thus, we ask annotators to label both API documentation blocks and the context dependence of each sentence.
Specifically, annotators cluster consecutive sentences that are context-dependent as a \emph{\textbf{S}emantic \textbf{U}nit} (SU). 
% Note that, for \so answers, 
Sentences in the same SU are labeled with the same section label.
A context-free sentence itself is also considered an SU. 
%  We show an example in the table~\ref{tab:semantic_unit}. Table~\ref{tab:semantic_unit} presents two consecutive sentences in one answer to illustrate the usage of BatchNorm API in \pt. All of the sentences shed light on the function of BatchNorm1d API. However, if we consider labeling individual sentences without context, the $sent_{2}$  should be less insightful as an explicit sentence subject is needed.
% Meanwhile, if we label sentences by considering their context but do not treat them as a semantic unit, the $sent_{2}$ should be labeled as insightful but may lose their context in the summarization stage, which would hinder the readability of the summary.
% Thus, regarding both $sent_{1}$ and $sent_{2}$ as a semantic unit is desired.
In other words, the output of the first labeling stage is a list of SUs labeled with the API documentation section.
% , which is different from prior work~\cite{chengran2022answer}.
% Specifically, for \so answers, we put multiple sentences into the same semantic unit if they meet the below criteria: 1) they are consecutive and located in the same paragraph; 2) sentences are semantically relevant (e.g., the subsequent sentence contains indicative pronouns); and 3) they have the same specification labels. We apply very similar criteria for video captions, while we consider only sentences in the same video rather than the same paragraph.
We explain our detailed labeling process below.

More specifically, following prior studies~\cite{uddin2017automatic, uddin2019automatic}, the whole labeling process consists of 3 steps:\newline
\textbf{Step I: Iterative Guideline Refinement.}
In each iteration, p1 and p2 independently label the same AU, which is randomly sampled from all AUs.
At the end of each iteration, a Cohen's kappa value is calculated. 
Then p1 and p2 discuss the sentence labels in disagreement jointly with a1. 
Then a1 refines the guideline based on the discussion and sends a new AU as well as an updated guideline to p1 and p2 for iterative labeling.
p1 and p2 repeat this process until the Cohen's kappa value reaches a substantial level of agreement (i.e., 0.62).\footnote{We interpret kappa values 0 as poor agreement, 0.01–0.20 as slight agreement, 0.21–0.40 as fair, 0.41– 0.60 as moderate, 0.61–0.80 as substantial, and 0.81–1.00 as almost perfect agreement.\cite{chengran2022answer,mantyla2015rapid}}
In total, 4 AUs are used for the guideline refinement step and dropped from \bench. 

% Then we perform full labeling, which is followed by validation labeling.
% % guideline refinement. , 2) full labeling, and 3) validation labeling phases.
% In particular, we use the Kappa coefficient~\cite{cohen1960coefficient} to measure the inter-annotator agreement.
% classify them into relevant API documentation blocks or the API-irrelevant class.
% Meanwhile, we consider clustering consecutive sentences that are semantically relevant as one semantic unit.  
% We follow the insight definition with Treude et.al~\cite{treude2016augmenting}, which claims an insightful sentence as sentences relevant to a specific API as well as providing insights that are not contained in the API document. 
% Different from Treude et.al~\cite{treude2016augmenting}, who treat the task as a binary classification that identifies whether one sentence is insightful or not, we aim to further classify insightful sentences into API document specifications (i.e., functionality, input\&output, and others), which is drawn from Java specification\footnote{https://www.oracle.com/java/technologies/javase/api-specifications.html}. 
% By doing so, each sentence directly maps to a specific document specification, which enables augmenting the API document on the specification level. We give the definition of each API specification below:
% \begin{itemize}
%     \item \textbf{Functionality}: Sentences that specify the expected or desired behavior of this API function, as well as its state transitions. When particular algorithms are leveraged in this API, specify the algorithm used in this operation.
%     \item \textbf{Input \& Output} Sentences that specify the behavior/range/algorithm of argument and return.
%     \item \textbf{Others} Sentences that contain other insightful tips to support developers better understanding and using the API (e.g., API performance, legal concern, and classic usage scenarios).
% \end{itemize}




% \noindent \textbf{Iterative Guideline Refinement.}
% Note that we discard labeled data (3 annotation units) with a low agreement (i.e., which Kappa value is lower than 0.6) in this collaborative labeling process and keep the labeled data in the last round of labeling. 

% Finally, we use the latest version of the guideline for full labeling.

% \begin{table}[]
%     \centering
%     \caption{Cohen Kappa value Interpretation}
%     \begin{tabular}{l|c}
%         \toprule
%         Kappa Value & Interpretation \\
%         \midrule
%         -1 -- 0     & poor           \\
%         0 -- 0.2    & slight         \\
%         0.2 -- 0.4  & fair           \\
%         0.4 -- 0.6  & moderate       \\
%         0.6 -- 0.8  & substantial    \\
%         0.8 -- 1.0  & perfect        \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:cohenkappa}
% \end{table}

\noindent\textbf{Step II: Full Labeling.}
a1, s1, and s2 label the remaining 16 AUs in the full labeling process after reading the final guideline.
In total, we label 4,344 sentences with API documentation sections in the first labeling stage.
% All labelers label with the latest updated version of the guideline.
% Annotators can contact the first author for further clarifying the guideline via   Teams during the full labeling stage. 
% In total, annotators label 4,344 sentences with API documentation blocks.
% Finally, annotators craft a sentence specification dataset including 4,344 sentences.
% , of which 2,134 are \so answer sentences and 2,210 are YouTube video caption sentences, respectively.

\noindent\textbf{Step III: Validation Labeling.}
% \red{haven't do it}
To perform validation labeling, we randomly sample 654 sentences from the full labeling data (i.e., 15\%).
a1 labels the sampled sentences independently to assess the data quality.
% The first author performs random sampling and selects a  subset of labeling objectives (i.e., 654 sentences). 
% 326 sentences and 328 sentences are selected with a 5 percent confidence interval for \so data and YouTube video captions, respectively. 
The kappa score between the annotators in the full labeling stage and a1 achieves a substantial level of agreement (i.e., 0.61), which illustrates that the quality of the API section classification data is high.
% \red{here we need to analyze the agreement between me and the labelers. waiting for the labeling result.}
% \red{here is the statistic for the sentence specification benchmark. waiting for the data.}
% \begin{table}[]
%     \centering
%     \caption{Semantic Unit Example}
%     \begin{tabular}{c|l}
%         \hline
%         Sentence & Content                                                         \\
%         \hline
%         Sent\_1  & BatchNorm has two "modes of operation": one is for training ... \\
%         Sent\_2  & The other "mode" is for evaluation: ...                         \\
%         % Sent\_3 & In this mode there is no problem processing samples one by one.\\
%         \hline
%     \end{tabular}
%     \label{tab:semantic_unit}
% \end{table}

\subsubsection{Phase 2: Update Summarization}
In the second phase, given a set of SUs associated with each API documentation section, annotators select SUs and form a summary.
Under a budget of selecting at most five SUs,
annotators rank and select SUs based on 1) the importance of each SU to understanding the API, 2) the clarity of each SU, 3) the redundancy among SUs, and 4) the redundancy between each SU and API document.  
% Each annotator is required to read the original API document page before labeling. 
Annotators are required to perform a greedy sentence selection~\cite{chengran2022answer} to remove sentences that are redundant to each other and redundant to the original API document.
They are allowed to select fewer than five SUs to form the summary if the number of SUs satisfying the above condition is less than five.
Phase 2 uses the same AUs and invites the same annotators in guideline refinement step and full labeling step as Phase 1.
Finally, 48 ($16 APIs \times 3 sections$) summaries are produced. 


% There is a special case for API `onPause'. 
% There is no SU associated with the input \& output block of this API.

% Since API `onPause' has no parameter, there is no sentence associated with the parameter block and thus the summary for the input \& output block is empty.

% To make annotators equip a consensus, we then follow TechSumBot to arrange meetings with annotators and provide labeling examples (excluded from the benchmark) to illustrate the overall labeling process.
%  Annotators are also available to contact the first author for clarifying the labeling process and guideline details via Teams. 

\subsection{Benchmark Statistics}
In \bench{}, the first phase data consists of 4,344 labeled sentences labeled with API documentation sections or irrelevant to the API. 
Each sentence is related to one of the 16 sampled APIs. 
The scale of the dataset is on par with previous related work~\cite{uddin2017automatic}.
The second stage data consist of 48 summaries, each of which is created from the first stage data.
The average SU number of the second stage input for each section (i.e., function, input \& output, and tips) is 18.76, 4.33, and 11.08, respectively.
% For each API, we further generate three summaries corresponding to three API documentation blocks (i.e., function, input \& output, and tips). 
The average number of SUs in the generated summaries of each section is 4.69, 2.77, and 4.31.
The summaries for the API function section have the highest compression ratio.
% Besides, we statistics the proportions of sentences from \so answers and YouTube video captions in the generated summary. 
On average, 20.51\% of SUs in the generated summaries are from YouTube video captions, while 80.12\% are from Stack Overflow answers. 
This indicates that the information in YouTube videos can effectively supplement \so in the API documentation augmentation task, while \so is still considered the primary resource for augmentation.
% Specifically, the average number of sentences for summaries related to each block type is 7.85, 3.77, and 6.38. 
% Since the number of sentences for summaries related to input \& output block is less than 5, it illustrates that 


% relevant to 16 APIs, in which sentences are labeled with API specifications. For each API specification, we further produce an extractive summary with a budget of at most five semantic units. In total there are 47 summaries exist (one API's specification does not have insightful sentences.)

% \red{to do list: 1) statistic of sentence num \& work num of each summary; 2) proportion of insightful sentences from \so answers and youtube video as well as the proportion in each specification (each specification expect to have different distribution to illustrate why multi-resource is helpful) 3) proportion of sentences from \so answer and youtube videos in the final summary 4) propotion of sentence context to prove the necessity context-awareness design}

==> chatgpt.tex <==
\red{a rough comparison to chatgpt}

\textcolor{red}{This section briefly talks about the reason for using extractive summarization rather than abstractive summarization in this task.
The logit is : we try to use ChatGPT to generate API summaries but failed due to trustworthy and vulnerability issues -> thus we use an extractive summarization framework to avoid the above drawbacks.}

\textcolor{red}{The main reason comes from the uncertain and commonly low factual consistency of the abstractive summarization approach. As the summary generated from the abstractive summarization model relies on the model's understanding, it is hard to guarantee the factual consistency of the generated summaries.}

In API summarization and recommendation tasks\red{citations about API ambiguity}, one crucial threat is API ambiguity as multiple API libraries may have the same name APIs with different usages or parameters. We expect that generate API summaries \textbf{would not incorrectly mention the information of the same name API in the other API libraries}. 

Thus, we perform a quantitative analysis on the state-of-the-art algorithm ChatGPT. We quantitatively explore whether ChatGPT would generate API summaries that involve incorrect information, especially the information from the API documentation of the same API name but different API libraries. 

Specifically, we are mainly interested in two scenarios: 1)whether the summaries generated by the abstract summarization model (e.g., ChatGPT) explicitly contain the information from incorrect API libraries, and 2)whether theose summaries would be misdirected by the incorrect prompt. 

As the APIs of the same name from different libraries commonly have different parameters, we can easily observe the factual consistency of API parameter summaries.
Therefore, we randomly select one API from \bench (i.e., Adadelta) as an example and design two prompts for generating the API parameter summaries to explore the factual consistency of the API summaries generated from the abstractive summarization model:
\begin{itemize}
    \item Prompt 1: give a summary of Adadelta's parameters in Pytorch.
    \item Prompt 2: what is use\_ema in Pytorch Adadelta API.

\end{itemize}
\noindent For the second prompt, note that the `use\_ema' parameter is only available in the Adadelta API document from the TensorFlow API library.\footnote{\url{https://www.tensorflow.org/api_docs/python/tf/keras/optimizers/experimental/Adadelta}} Adadelta API in \pt (version: 1.13) has not implement such parameter.\footnote{https://pytorch.org/docs/stable/generated/torch.optim.Adadelta.html} We aim to explore whether the summary from ChatGPT would involve incorrect information due to a misleading prompt (i.e., ask the model to generate a summary for a Pytorch API parameter that actually do not exist). 
Surprisingly, we find that the generated summaries from both prompts contain obvious factual errors. 

\textbf{Result of Prompt1}
The ChatGPT-generated summary from the first prompt is shown in Figure~\ref{fig:1stprompt}, which gives a brief summary of the Pytorch API Adadelta's parameters.

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figure/prompt_1.png}
    \caption{Summary from the First Prompt }
    \label{fig:1stprompt}
\end{figure}

We highlight two obvious factual inconsistencies in the red boxes. There is no parameter `amsgrad' and `max\_grad\_norm' in Pytorch's Adadelta API. Actually, AMSgrad is an optimizer modified from the Adam optimizer algorithm. Thus `amsgrad' serves as a parameter in Adam\footnote{https://pytorch.org/docs/stable/generated/torch.optim.Adam.html?highlight=amsgrad} and AdamW in \pt. 
As Adadelte, Adam, and AdamW are all algorithms for optimizers, we assume that ChatGPT is hard to distinguish APIs that have similar usage but from different API libraries and thus produce inaccurate summaries. We further randomly sample 5 APIs and ask ChatGPT to produce parameter summaries with similar prompts, 4 out of 5 contain incorrect parameters, which highlights the trustworthy issue of ChatGPT.  

Note that we can not even find a \pt API document that mentions `max\_grad\_norm' parameter (from version 0.1.12 to version 1.13 as listed in \pt official website). The most relevant parameter is the `max\_norm' in \pt's `torch.nn.utils.clip\_grad\_norm\_' API, which is used to set the max norm of the gradients (the usage is the same as which in ChatGPT's summary). Meanwhile, we find the same parameter name occurs in some APIs with different usage from Hugging Face (e.g., Trainer\footnote{\url{https://huggingface.co/transformers/v3.5.1/main_classes/trainer.html}}) and Apex (e.g., FusedLAMB\footnote{\url{https://nvidia.github.io/apex/optimizers.html}}) libraries. This observation indicates that ChatGPT may summarize other API libraries' information even the usage of those APIs is different from the prompted APIs.   

\textbf{Result of Prompt2}
The ChatGPT-generated summary from the second prompt is shown in Figure~\ref{fig:2ndprompt}, which attempts to give a summary for the `use\_ema' parameter in \pt's Adadelta. Note that `use\_ema' actually does not exist in the \pt document and only occurs in the TensorFlow API document.

\begin{figure}
    \centering
    \includegraphics[width=1\columnwidth]{figure/prompt_2.png}
    \caption{Summary from the Second Prompt }
    \label{fig:2ndprompt}
\end{figure}

As shown in Figure~\ref{fig:2ndprompt}, ChatGPT does generate a summary for an Adadelta parameter that actually does not exists in \pt document. 
As `use\_ema' is described in Tensorflow's Adadelta API document, we further manually compare the semantical similarity between ChatGPT generated summary and the corresponding description in the Tensorflow API document.\footnote{\url{https://www.tensorflow.org/api_docs/python/tf/keras/optimizers/experimental/Adadelta}} We empirically find that this ChatGPT generated summary perfectly covers all information in the Tensorflow API document. 
ChatGPT seems to be vulnerable to API ambiguity and considers the API information with the same name but in different libraries as the ground truth.
We further build similar prompts for five other randomly sampled APIs from Pytorch against TensorFlow and observe the same result. 
Though OpenAI claims that ChatGPT is optimized and thus available to challenge incorrect premises and reject inappropriate requests\footnote{\url{https://openai.com/blog/chatgpt/}}, our quantitative analysis finds that ChatGPT's output for API summarization is possibly misleading by the prompts that misuse a parameter not existing in the original document, which highlights the vulnerability of ChatGPT on API summarization.

Overall, we highlight that ChatGPT has vulnerability and trust-worthy issues. Specifically, ChatGPT is hard to distinguish APIs in the API summarization task that has the same name but from different API libraries or APIs with similar usage. Sometimes it even leverages the knowledge from irrelevant APIs from different API libraries. Finally, ChatGPT is vulnerable to fake API parameters drawn from non-target API libraries. 

To our best knowledge, there is no existing large-scale API summarization benchmark for training API summarization generation models and optimizing for the aforementioned drawbacks, thus generating API summaries must rely on text generation models trained from large general-domain datasets. 
However, through our quantitative analysis, we find that the state-of-the-art text generation tool ChatGPT suffers from vulnerability and trust-worthy issues, which making ChatGPT not suitable for API document summarization task as the high priority for the correctness of API information\red{citation to unveiled API document}. 
To mitigate the vulnerability and trust-worthy issues, we tend to implement an extractive-based summarization framework, which ranks and selects sentences from multiple information sources to guarantee that the chosen sentence remains identical to the original resource.

==> dataconstruct.tex <==
\label{benchmark}


We present \bench{}, the first Stack Overflow multi-answer summarization benchmark for answering a specific technical question.
% \bowen{We'd better provide the definition of ``annotation unit'' at the beginning of this section rather in any subsection.}
% \bowen{The following sentence sound like we start with 37 queries which is a odd number. Instead, we should say something like ``we start with 50 annotation units. 10 of them are used for pilot study and the rest 40 are fed to the labeling process. Among those 40 units, 3 of them are removed due to the low agreements. As a result, we build \bench{} with 37 technical queries at the end.''}
Figure~\ref{fig:bench_diagram} describes our benchmark construction process. We firstly automatically collect \emph{annotation units}, which is then followed by the data cleaning process described in Section~\ref{sec:datacollection}.
An annotation unit consists of a technical question and multiple relevant answers.
Next, six annotators perform a two-phase labeling process: useful sentence selection and summary generation as explained in Section~\ref{sec: labelingprocess}. 
Note that we perform an iterative guideline refinement for the useful sentence selection task until the inter-annotator agreement achieves a certain level as described in Section \ref{sec: useful sentence selection}. 
% In the full labeling process, 3 annotation units are removed due to the low inter-annotator agreement. As a result, we build \bench{} with 37 technical queries and 111 query-summary pairs.

% \bowen{Write a paragraph about participants information here}





\subsection{Data Collection}\label{sec:datacollection}
We prepare 50 annotation units (i.e., technical query and multiple relevant answers) by performing automatic data extraction and data cleaning.


\subsubsection{\textbf{Automatic Data Preparation}}\label{automatic_data}

The PostLinks table in \so{} data dump\footnote{\url{https://archive.org/details/stackexchange}} contains the information of user-voted duplicated question links, in which each original question is linked to their duplicated questions.
% We refer the earliest published \so{} questions to the original questions.
Specifically, an original question refers to the earliest published \so{} question that is a duplicate of newer questions. The duplicate questions\footnote{https://stackoverflow.com/help/duplicates} are manually marked by following a strict mechanism that one moderator or at least three active users (i.e., users who have over 3,000 reputation score) vote the questions to be a duplicate to the original one. 
% To select technical questions and their corresponding ground-truth answers from \so,
% rather than manually selection, we leverage the information of duplicated post links from \so datadump to automatically extract them. 
In particular, we treat the title of the original question as the technical question of each annotation unit in \bench{}. As the \so{} questions with `duplicate' links are labeled by reputable \so{} users, we regard all the answers to the original question and their duplicates as the relevant answers of the technical question in the corresponding annotation unit. 

To prepare the labeling materials, we randomly extract 50 annotation units from the PostLinks table in Stack Overflow data dump. %duplicated post links by considering some criteria. 
We focus on questions related to two popular programming languages, Python and Java, by checking if they are tagged with `Java' or `Python'. 
% Since these languages are popular, it alleviates the threat that annotators are not familiar with each answer's background knowledge and mistakenly annotate.
Following AnswerBot~\cite{xu2017answerbot}, we only consider the technical questions in which the sum of the number of answers is between 10 to 15. We discard answers with no vote as their usefulness to the technical question is unclear or considered as bad by \so{} users. As we focus on the text summarization, answers that only contain code snippets without text content are also dropped.


% \begin{table}[]
%     \centering
%     \caption{Semantic Gap between Question Title and Description}
%     \begin{tabular}{c|p{5cm}}\hline
%         Question Title  & \textbf{\#17027777}: Relationship between hashCode and equals method in Java \\ \hline
%         Question Description &\textbf{\#17027777}: I read in many places saying while \textbf{override \textit{equals} method in Java, should override \textit{hashCode} method too}, otherwise it is "violating the contract". 
%         % But so far I haven't faced any problem if I override only equals method, but not hashCode method. 
%         ...
%         What is the contract? And why am I not facing any problem when I am violating the contract? In which case will I face a problem if I haven't overridden the hashCode method?\\ \hline
%         Example Answer & \textbf{\#10143020: \textbf{Yes, it should be overridden.} If you think you need to override equals(), then you need to override hashCode() and vice versa...}\\ \hline
%     \end{tabular}
%     \label{tab:semantic gap}
% \end{table}

% \subsubsection{\textbf{Manual Data Filtering}}
% \cran{this section may not necessarily to present}
% To ensure the answers in the \bench{} answer the technical question, we filter out the \so posts whose question titles has a semantic gap with their question descriptions. 
% % We observed that, for some \so{}question posts, there is semantic gap between the question title and the corresponding detailed description. 
% Table \ref{tab:semantic gap} provides a concrete example. The question title queries the general relationship between two methods in Java while the question description only focuses on the `override contract' aspect. We observe that the answers usually focus on the detailed question description, which leads the answer away from the question itself.
% % answers but only serves as the subset of expected answer to the question itself. 
% For instance, the example answer in Table \ref{tab:semantic gap} only focus on the consistency of both methods on `override' aspect, which should not be regarded as a satisfactory answer to the question.
% %We prepare 50 annotation units for labeling, in which 10 for pilot labeling process and 40 for full labeling process. We describe the detailed labeling process in Section \ref{labelingprocess}.
% We exclude questions with such semantic gap.
% To achieve this, one author of this study randomly selects one annotation unit at a time from the result of \textit{automatic data extraction} stage and performs manual check. Another author then double-check each annotation and identify whether selected ones meet the above requirement. If there are annotation units that do not meet the requirement, we discard them and collect more annotation units until we have 50 annotation units without the semantic gap. 
% \vspace{-2mm}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=8.5cm]{figure/benchmark_diagram_v2.pdf}
    \vspace{-6mm}
    \caption{Benchmark Construction}
    \label{fig:bench_diagram}\vspace{-4mm}
    % \bowen{the figure needs to be updated}
\end{figure}



\subsubsection{\textbf{Data Cleaning}}
We pre-process the 50 annotation units. We use NLTK\footnote{https://www.nltk.org/api/nltk.tokenize.html} to break each text content into sentences. 
We then apply some heuristics to reduce noise. 
We exclude sentences that consist of only an external hyperlink since the hyperlink content is not directly visible. 
For sentences that consist of both hyperlinks and text content, we keep the text content and replace the hyperlinks with a place holder (i.e., `[external-link]').  
We also replace the code snippet, table and pictures in answers with place holders (i.e., `[code-snippet]', `[table]', `[figure]'). Additionally, we observe that the inline code is important for annotators to understand the sentence meanings. Therefore, we keep the inline code. 
Furthermore, we treat multi-level headings which is more than five words in answers as individual sentences as we observe that they are frequently summative sentences.
Finally, each annotation unit after the above pre-processing serves as the labeling materials. 
% \textcolor{blue}{Table shows an annotation unit example.} 
% \cran{Do we need a example here?}
% \vspace{-2mm}
\subsection{Labeling Process}
\label{sec: labelingprocess}


Firstly we prepare labeling materials for annotators to get ready for the labeling process.
We present the content of each annotation unit into a text file that contains the technical question, sentences from each answer, \so{} hyperlinks to each answer, and a blank section for labeling. Each answer sentence is assigned with a unique identifier based on its source answer and the sentence order in the source answer. For example, the fourth sentence in the third answer of the annotation unit is assigned with the identifier $\#03\_04$. We also provide the guideline.

Then we follow a two-phase labeling process that is commonly used in NLP studies \cite{angelidis2021extractive, angelidis2018summarizing}. 
Six annotators are involved in the labeling process.
% \bowen{basic info (like programming experience) about participants (why they are qualified/knowledgeable for the labeling task) is missing here. something similar to Section 5.2}
All participants are PhD students and have at least two years of development experience in Java and Python programming languages.
In each phase, annotators and labeling materials are divided equally into two groups. Three participants in one group label the same group of labeling materials. 
The goal of the labeling process is to select summative sentences from multiple answers to form a brief summary of answers to a technical question.
To achieve this, in the first phase (i.e., \textit{useful sentence selection}), three annotators select the useful sentences from all relevant answers.
The sentences that all annotators agreed to be useful for answering the technical question serve as the input of the second phase (i.e., \textit{summary generation}).
In the \textit{summary generation} phase, three annotators are asked to select five sentences that will form an extractive summary based on the sentences' clarity, redundancy and importance. In prior summarization works from NLP field, it is common to select a fixed number of sentences~\cite{parveen2015topical, liu2019text, zhong2020extractive} , e.g., five sentences~\cite{parveen2015topical, zhong2020extractive}, as the summary.

\vspace{-3mm}
\subsubsection{\textbf{Phase 1: Useful Sentence Selection}}\label{sec: useful sentence selection}
In this labeling stage, annotators are required to identify the useful sentences for answering the technical question from multiple \so{} answers. 
The labeling objective is formulated as a binary classification that specifies sentence usefulness to the technical question. 
Annotators label the sentences for answering the technical question as either `useful' or `not-useful'. Sentences are labeled as `?' when annotators are unsure whether the sentences are useful to answer the question. Note that we do not consider the redundancy among sentences in this phase. 
% Furthermore, we observe some labeling rules that may improve the inter-annotator agreement when performing pilot labeling. 
% % \textcolor{blue}{We summarize those labeling rules in the guideline and apply them on full labeling process.}
% % \cran{not sure whether we summarize the rules here or we provide a hyperlink to guideline from the github repo}
% \textcolor{blue}{We summarize the labeling rules. Firstly, though annotators can use context information to understand each sentence, they are required to identify the usefulness of each sentence independently. Besides, general comments about the query itself or solutions should often be avoided (e.g., 'I hate Java!''), as they don't provide further useful information to answer the query. Finally, for those sentences that aren't complete, annotators aren't allowed to assume the usefulness of hidden parts (e.g., 'The above code can answer your question:').}
In particular, we use the Kappa coefficient \cite{cohen1960coefficient} to measure the inter-annotator agreement. A higher kappa value illustrates a higher agreement level among annotators. We follow prior studies~\cite{joblin2017classifying, lee2017understanding,mantyla2015rapid} to interpret the meaning of Kappa value: kappa values 0 as poor agreement, 0.01–0.20 as slight agreement, 0.21–0.40 as fair, 0.41– 0.60 as moderate, 0.61–0.80 as substantial, and 0.81–1.00 as almost perfect agreement.



% \begin{table}[!htbp]
%     \centering
%     \caption{Kappa Agreement Levels}
%     % \resizebox{\linewidth}{}{
%     % \begin{tabular}{c|C{1cm}C{1cm}C{1cm}}
%     \begin{tabular}{c|c}
%     \toprule
%     Kappa Statistic & Agreement Level     \\
%     \midrule
%     <0.00 & Poor\\
%     0.00-0.20 & Slight\\
%     0.21-0.40 & Fair\\
%     0.41-0.60 & Moderate\\
%     0.61-0.80 & Substantial\\
%     0.81-1.00 & Almost Perfect\\
%     \bottomrule
%     \end{tabular}\\

%     \label{table: kappa}
% \end{table}

\noindent\textbf{Iterative Guideline Refinement} To ensure the quality of the selected useful sentences, we performed an iterative guideline refinement to improve the inter-annotator agreement, which is widely adopted in the literature~\cite{chang2017revolt, sheng2008get}. Specifically, six annotators label the same annotation units in each iteration. In each round, we polish the guideline and update the labeling materials according to the annotator feedback and automatic evaluation result. 
We end the guideline refinement process when the inter-annotator agreement level is \textit{Moderate}. 
% We follow existing studies \cran{citation} to explain the meaning of Kappa value as shown in Table \ref{table: kappa}. 
The annotation units used in the guideline refinement process are discarded. Specifically, we discard 10 annotation units in the guideline refinement process
and have 40 annotation units for full labeling.

\noindent\textbf{Full Labeling Process} 
Firstly we arrange meetings with the annotators to align the understanding of the guideline. We share the labeling rules that are obtained while observing the guideline refinement process with annotators. In particular, annotators should identify the usefulness of each sentence independently of its context (e.g., surrounding sentences). 
Additionally, general comments about the question itself or its solutions should be avoided (e.g., ``I hate Java!''), as they do not provide useful information to answer the query. Finally, for incomplete sentences, annotators should not assume the usefulness of its hidden part (e.g., ``the content in `[code snippet]' place holder''). 

After the labeling process is finished, one author deals with the labeling results. In each annotation unit, all the sentences that three annotators agree to be useful to that question, coupled with the technical query, serve as the input to the second phase. 
Note that, there are three annotation units whose inter-annotator agreement is \textit{Slight} (i.e., the Kappa value $k$ is 0.00 $\leq$ $k$ $\geq$ 0.20) in the full labeling process. We consider a good agreement to be at least \textit{Moderate} (i.e., the Kappa value $k$ is 0.40 $\leq$ $k$ $\geq$ 0.60). Therefore, we discard these annotation units as the labels may not be of good quality. We have 37 sets of $\langle$ question, useful answers $\rangle$ pairs in total.  

\noindent\textbf{Inter-Annotator Agreement of Phase 1}
The average kappa value of the \textit{useful sentence selection} phase is 0.43, indicating the annotators achieve \textit{Moderate} agreement.
Previous work shows that the human agreements on sentence selection task for constructing news-domain summarization benchmarks are usually lower than 0.3 ~\cite{radev2003evaluation}. Additionally, the kappa value of a recent opinion summarization benchmark is 0.36~\cite{angelidis2021extractive}. It indicates that the inter-annotators agreement on sentence selection task in our \bench{} is comparable to those of common \nlp{} benchmarks. 

\vspace{-2mm}
\subsubsection{\textbf{Phase 2: Summary Generation}}

In the second phase, given a set of useful sentences to answer the technical question, annotators are required to generate a final extractive summary under a budget of five sentences by selecting sentences based on three key factors, i.e.,clarity of each sentence, redundancy among sentences, and the importance for each sentence to answer the question. 

% \begin{algorithm}
% \caption{Summary Generation}\label{alg:summarygeneration}
% \SetKwComment{Comment}{/* }{ */}
% \SetKwInput{KwInput}{Input}                % Set the Input
% \KwInput{T[]: List of answer sentences}
% % \KwData{$n \geq 0$}
% \KwResult{S[]: List of summary sentences}
% candidate\_list = [] \Comment*[]{initialize empty candidate list}
% summary\_list = [] \Comment*[]{initialize empty summary list}
% RC[0].append(T[0]) \Comment*[]{RC[i] refers to the ith Redundant Cluster}
% % result\_list[0] = T[0]
% % \For{$k=1$ \KwTo $n$}{
% % }

% \For{current \textbf{in} range(T)}{
% % \Comment*[l]{assign each sentence into RCs}
%     \For{ith RC \textbf{in} RC}{
%         % \;
%         \For{sent \textbf{in} ith RC}
%             {
%             \eIf{is\_redundant(sent, sent)}
%                 {RC[i].append(current)\Comment*[]{assign with the same RC}}
%                 {RC[len(RC)+1].append(current)\Comment*[]{assign with the new RC}}
%             }
     
    
%     }

% }

% \For{ith RC \textbf{in} RC}{
%     % \;
%     summative\_sent = select\_most\_summative\_sent(ith RC)\;
%     candidate\_list.append(summative\_sent)\;
% }

% % \eIf{len(result\_list) > 5}
% %     {delete_less_importance(result\_list, 5)}
% %     {add_important(result\_list, 5)}

% \eIf{len(candidate\_list) > 5}
%     {summary\_list = delete\_by\_importance(candidate\_list, 5)}
%     {summary\_list = add\_by\_importance(candidate\_list, 5)}

% return summary\_list

% \end{algorithm}

% \noindent\blue{\textbf{Quality Control Meeting}}

% \begin{table}[t]
% % \vspace{-3mm}
%     \centering
%     \caption{\bench{} Details}
%     % \resizebox{\linewidth}{}{
%     % \begin{tabular}{c|c{1cm}c{1cm}c{1cm}}
%     \begin{tabular}{l|l}

%     \toprule
%     Field &Description   \\
%     \midrule
%     \multicolumn{2}{c}{Technical Question}\\\hline
%     Question Title & Question Title in string\\
%     Question Id & SO Id for original post\\
%     Question Tags & SO Tags for original post\\
%     Question Link & SO hyperlinks to the original post\\

%     \hline\multicolumn{2}{c}{Summaries}\\\hline
%     Summary Id & Summary id \{1,2,3\}\\
%     Summary Body & Summary under a budget of five sentences\\
%     Source Answer Id & Id of source answers for making summary\\

%     \hline\multicolumn{2}{c}{Source Answer}\\\hline
%     Answer Id & SO Id for the answer post\\
%     Answer Body & List of sentences from the Answer\\
%     Answer Link & SO hyperlinks to the answer post\\

    
    
%     \bottomrule
%     \end{tabular}\\

%     \label{table: datafield}\vspace{-5mm}
% \end{table}


To let annotators equip a consensus of the goal, we arrange a meeting with all the annotators for two things.
First, we provide an example (excluded from the data used from constructing the benchmark) to demonstrate the materials and the brief overall labeling process.
Second, we let them align their understanding based on the materials by discussing with each other.

After that, annotators select sentences by following the process: first, all sentences are clustered into different RCs (Redundant Cluster) in which each sentence is semantically similar; then the annotator should select the most summative sentence with high clarity from each RC into the candidate list; finally the annotators are asked to delete sentences from the candidate list until only five sentences are left, by taking into account how well each sentence answers the question. 
Note that, for each group of sentences in our benchmark, there are always more than five RCs clustered by annotators.
Finally, the top five sentences serve as the summary of the answers to the technical question.





\vspace{-2mm}
\subsection{Benchmark Statistic}

% \begin{table}[htbp]
%     \centering
%     \caption{Statistic of \bench{}}
% \scalebox{0.93}{

%     \begin{tabular}[8cm]{cccc}\hline
%     \#Query& \#Summary & Avg.\#Word/Summary &Avg.\#Sent/Summary    \\\hline
%     37& 111 & 106.45 & 5 \\\hline
%     \end{tabular}}
%     \label{tab:statisticofbench}
%     % \bowen{add (1) how many words per ground truth sentence? (2) how big overlap between ground truth summaries?}
% \end{table}

% \blue{Table \ref{tab:statisticofbench} describes the \bench{} statistics. $\#$Word/Summary refers to the average number of words in ground-truth summaries. $\#$Sent/Summary refers to the average number of sentences in ground-truth summaries.
% \bowen{we provide basic information (url, content,etc) of all the included question, answer}
In \bench{}, there are 37 technical questions, each of which corresponds to three ground truth answer summaries that are independently labeled by three annotators. Each summary contains five sentences extracted from corresponding relevant answers.
In total, we have 111 query-summary pairs. The average number of words in ground-truth summaries is 106.45. 
The scale of \bench{} is comparable with two commonly used query-focused multi-documentation summarization benchmarks in the NLP community~\cite{dang2005overview, gao2021simcse}, i.e., DUC-2005 and DUC-2007, which consist of 50 and 45 annotation units, respectively. 
% We provide the meta data of question and answers (i.e., Id, Tags and url )
% We show the data fields of \bench{} in Table \ref{table: datafield}.

% \cran{Do we need further statistics, e.g., the ratio of the sentences in the final summary that originally comes from accepted/most vote answer? Or the avg number of sentences in each redundant cluster?}







==> plan.tex <==
\begin{itemize}
    \item Dec 29 - Nov 3
        \begin{itemize}
            \item Literature review
            \begin{itemize}
                \item context-awareness mechanism
                \item hierarchically model the importance of each sentence (sent \& word level) 
                \item supervised summarization (train with SOSUM dataset)
                \item update summarization algorithm
            \end{itemize}
            \item Approach implement
            \item Paper writing for Benchmark Section
            \item Continue crafting the benchmark
        \end{itemize}
    \item Nov 4 - Nov 9
        \begin{itemize}
        \item Approach implement    
        \item Paper writing for Approach and other sections except for Experiment result section
        \end{itemize}
    \item Nov 11 - Nov 17
        \begin{itemize}
            \item Approach implement
            \item Paper writing and modification 
        \end{itemize}
\end{itemize}

\subsection{approach}
Basically, we have two sub-module in our approach.

For the first module, given the relevant Stack Overflow answers and YouTube video captions, we identify the most important semantic units with respect to the specific API and classify them into three pre-defined aspects (i.e., basic, parameter, and others).

Given a list of semantic units in each aspect, the second module generates a summary while taking into account the redundancy between the generated summary and the ground-truth API document.
\subsection{dataset}
I'm not sure, but we may consider crafting a moderate-size dataset (like labeling 60 summaries for 20 APIs) in our first submission (in case the dataset is required to update).
\subsection{Evaluation}
For the first module, we evaluate via our dataset's first stage result in terms of Precision, Recall, and F1 score. We follow the setting of our SANER paper.
For the second module, we evaluate in both automatic and manual manners. For the automatic evaluation, we use Rouge to compare the similarity between the generated summaries and ground truth. For the manual evaluation, we follow the setting of our ASE paper. 
\subsection{Reminder}


==> threats.tex <==


